A Framework using Contrastive Learning for Classification with Noisy Labels

We propose a framework using contrastive learning as a pre-training task to perform image classification in the presence of noisy labels. Recent strategies such as pseudo-labeling, sample selection with Gaussian Mixture models, weighted supervised contrastive learning have been combined into a fine-tuning phase following the pre-training. This paper provides an extensive empirical study showing that a preliminary contrastive learning step brings a significant gain in performance when using different loss functions: non-robust, robust, and early-learning regularized. Our experiments performed on standard benchmarks and real-world datasets demonstrate that: i) the contrastive pre-training increases the robustness of any loss function to noisy labels and ii) the additional fine-tuning phase can further improve accuracy but at the cost of additional complexity.

==> sections/05_improvements.tex <==
\section{Details on the proposed improvements}

\subsection{Sample selection and sample correction with pseudo-labels}
Pseudo labels represent one hot encoded model's predictions on the training set. Temporal ensembling used in ELR is a technique to generate pseudo labels. Using pseudo-labels is a widespread technique both in semi-supervised learning and in noisy label classification. The former typically leverages the predictions of a model trained on a labeled subset to a larger unlabeled dataset. In the noisy label setting, various techniques (e.g. DivideMix, etc) identify a subset with a high likelihood of correctness and treat the remaining samples as the unlabeled counterpart in semi-supervised learning. In this work, we elaborate on the observation that the train-set labels predicted after training the model with a noise-robust loss function are more accurate than the ground truth. The quality of train-set predictions, denoted here pseudo labels, has been depicted in~\autoref{fig:pseudolabels}, which collects the results of all presented experiments on CIFAR 100. Pseudo labels are more accurate than the corrupted ground truth for both symmetric and asymmetric noise and bring a higher gain in performance as the noise ratio increases.
\begin{figure}[h]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/pseudolabels.pdf}}
\caption{ Accuracy of pseudo labels on symmetric (a) and asymmetric (b) noise has been evaluated on CIFAR 100. In all cases the pseudo-labels have a higher accuracy than the corrupted ground truth and the gain increases with the noise ratio}
\label{fig:pseudolabels}
\end{center}
\vskip -0.2in
\end{figure}

Optionally, as proposed by other state-of-the-art approaches, the loss value on train samples can be used to discriminate between clean and mislabeled samples. As proposed in DivideMix~\cite{li2020dividemix}, a sample correctness probability can be computed by fitting a 2 components GMM model on the distribution of losses and using the underlying probability as a sample weight:
\begin{equation}
    w_i  = p(k= 0|l_i).
\end{equation}
~\autoref{fig:sample_weighting} depicts the evolution of the clean train set identified using the GMM selection on CIFAR100, when the ground truth accuracy is 20\%. Its accuracy increases from 0.3 to 0.5 while its size reduces from 60\% to 30\%.
\begin{figure}[h]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/sample_weighting.pdf}}
\caption{ Clean train set accuracy (a) and size (b). The clean train set consists of all samples with small loss values, identified as the membership probability to a 2 components GMM.}
\label{fig:sample_weighting}
\end{center}
\vskip -0.2in
\end{figure}


\subsection{Supervised contrastive learning with weighted samples}
Supervised contrastive learning~\cite{khosla2020supervised}.
The author propose a simple modification to the contrastive loss function defined in~\autoref{eq:contrastive_loss} to leverage label information:
\begin{equation}
    L_i = -log\frac{1}{|P(i)|} \sum_{p \in P(i)}\frac{exp(\bm{z_i}^T \bm{z_{p}}/ \tau)}{\sum_{a\in A(i)}exp(\bm{z_i}^T \bm{z_a}/ \tau)},
    \label{eq:supervised_contrastive_loss}
\end{equation}
where $P(i) = \{ I \setminus \{i\}, y_i = \widetilde{y_i}  \}$ with $\widetilde{y_i}$ the prediction of the model for input $\bm{x_i}$. 

As explained in the previous section, the loss value for the training set samples was used to fit a Gaussian Mixture model with 2 components, corresponding to correctly and incorrectly labeled samples. The underlying probability $w$ of membership to the correctly labeled component was employed as a weighting factor in the supervised representation phase. Thus, likely mislabeled samples, having large loss values would contribute only marginally to the supervised representations:
\begin{equation}
    L_i = -log\frac{1}{|P(i)|} \sum_{p \in P(i)}\frac{\widetilde{w_{p,i}} exp(\bm{z_i}^T \bm{z_{p}}/ \tau)}{\sum_{a \in A(i)}exp(\bm{z_i}^T \bm{z_p}/ \tau)},
    \label{eq:supervised_contrastive_loss_weighted}
\end{equation}
where $\widetilde{w_{p,i}}$ is a modified version of $w_p$ such as $\widetilde{w_{p,i}} = 1$ if $p = j(i)$ else $\widetilde{w_{p,i}}= w_i$. If all samples are considered as noisy,~\autoref{eq:supervised_contrastive_loss_weighted} is simplified into the classical unsupervised contrastive loss in~\autoref{eq:contrastive_loss}.

\subsection{Dynamic bootstrapping with mixup}
The weights $w$ computed by the sample selection phase can also be combined with a mixup data augmentation strategy~\cite{Zhang2018mixup}. A specific strategy for noisy labels, called dynamic bootstrapping with mixup~\cite{arazo2019unsupervised}, has been developed to help convergence under extreme lavel noise conditions. The convex combinations of sample pairs $x_p$ and $x_q$ is weighted by the probability $w$ to belong to the clean dataset:
\begin{equation}
    x = \frac{w_p} {w_p + w_q}x_p + \frac{ w_q}{ w_p + w_q }x_q.
\end{equation}
The associated CE is corrected accordingly to the weights:
\begin{equation}
l_{ce b}(\theta) = - \sum_{i=1}^{N} (w_i y_i + (1-w_i) z_i)^T log(h_\theta(x_i)),
\end{equation}
where $z_i = \argmax (f_\theta(\bm{x_i}))$. If the GMM probability are well estimated, combining one noisy sample with one clean sample leads to a large weight for the clean sample and a small weight for the noisy sample. Clean-clean and noisy-noisy cases remain similar to a classical mixup with weights around $0.5$.

The dynamic bootstrapping can also be derived for the ELR:
\begin{equation}
l_{elr}(\theta) = l_{ceb}(\theta) + \frac{\lambda_{elr}}{N} \sum_{i=1}^{N} log \left( 1 - \langle p^i, t^i \rangle 	\right) 
\end{equation}

And for the robust loss function NFL+RCE:
\begin{equation}
\begin{aligned}
    & l_{nfl} =  w \frac{ -\sum\limits_{k=1}^{K} q(k|x) (1-p(k|x))^\gamma log(p(k|x))}{-\sum\limits_{j=1}^K \sum\limits_{k=1}^{K} q(y=j|x) (1-p(k|x))^\gamma log(p(k|x))} \\
    & + (1 - w) \frac{ -\sum\limits_{k=1}^{K} z(k|x) (1-p(k|x))^\gamma log(p(k|x))}{-\sum\limits_{j=1}^K \sum\limits_{k=1}^{K} z(y=j|x) (1-p(k|x))^\gamma log(p(k|x))}
\end{aligned}
\end{equation}
where $q$ is the one-hot encoding of the label (the zero value is fixed to a low value to avoid $log(0)$).
\begin{equation}
    l_{rce} = -\sum_{k=1}^{K} p(k |x)log \left( w. q(k | x) + (1-w)z \right)
\end{equation}

\iffalse
\subsection{Framework coupling robust learning and self-supervised learning}
As illustrated in~\autoref{fig:full_workflow}, the full workflow is composed of two blocks: pre-training+pseudo-labels and improvements. Each block has a classification phase preceded by a contrastive learning phase. As explained in the previous section, the first block generates pseudo-labels for the second block. The second block leverages the improved labels to perform a sample selection by fitting a 2 components GMM model on the distribution of losses and using the underlying probability as a sample weight.


 sample correctness probability can be computed 
its good reputation to attract customers.


Overview of the proposed method. A process consisting of two blocks (pre-training/pseudo-labels and improvements) is proposed: the first one produces train-set pseudo labels $\widehat{y}$ and the second used the pseudo labels $\widehat{y}$ as a new ground truth. Each step is preceded by a contrastive pre-training, in an unsupervised way for the first block and in a supervised way for the second block, leveraging the predicted pseudo labels to generate the final predictions $\widehat{y}_{final}$.







In this experiment, we combined two classification phases performed with noise-robust losses. The goal of the first phase was to produce optimized train-set pseudo labels while the second one used the pseudo labels as the new target variable. The pseudo labels represent one hot encoded model's predictions on the train-set. Other techniques to generate pseudo labels have been explored, as detailed in the next section (e.g. temporal ensembling as proposed in ELR). Optionally, as proposed by other state-of-the-art approaches, the loss value on train samples can be used to discriminate between clean and mislabeled samples. As proposed in DivideMix, a sample correctness probability can be computed by fitting a 2 components GMM model on the distribution of losses and using the underlying probability as a sample weight.
%\begin{figure}[ht]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=\columnwidth]{figures/method.png}}
%\caption{ Overview of the proposed method. A process consisting of 2 classification phases (b and d) is %proposed: the first one produced train-set pseudo labels and the second used the pseudo labels as a new ground %truth. Each classification phase is preceded by a contrastive pretraining, in an unsupervised setting for (a) %%and in a supervised way for the (c), leveraging the predicted pseudo labels.}
%\label{fig:method}
%\end{center}
%\vskip -0.2in
%\end{figure}

Each of the two classification phases is preceded by a representation learning phase, using contrastive methods. The following self-supervised representation frameworks have been compared: Simclr, Moco, Mopro. As depicted in Figure 3, representation phases update the network up to the classification heads (depicted in blue). Some methods (e.g. Moco) employ an additional projection head (illustrated in yellow). The first representation learning step was performed in an unsupervised setting, as proposed in the original works. The second representation phase (Figure 2, c) ran in a supervised setting using the pseudo labels and optionally, the computed sample weights. 

%\begin{figure*}[ht]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=2.0\columnwidth]{figures/network.png}}
%\caption{ Network architecture. Our experiments used ResNet models having as classification head either a linear layer (in red, panel a) or 2 stacked fully connected layers, setting referred to as multilayer (in red, panel b). The classification head follows the representation layer (the last resnet fully connected layer). The representation learning phase uses projection heads, connected to the representation layer, consisting of either a linear layer (in yellow, panel a) or multiple layers (in yellow, panel b).}
%\label{fig:network}
%\end{center}
%\vskip -0.2in
%\end{figure*}

\fi
